Manifold Coordinates with Physical Meaning

Manifold embedding algorithms map high-dimensional data down to coordinates in a much lower-dimensional space. One of the aims of dimension reduction is to find intrinsic coordinates that describe the data manifold. The coordinates returned by the embedding algorithm are abstract, and finding their physical or domain-related meaning is not formalized and often left to domain experts. This paper studies the problem of recovering the meaning of the new low-dimensional representation in an automatic, principled fashion. We propose a method to explain embedding coordinates of a manifold as non-linear compositions of functions from a user-defined dictionary. We show that this problem can be set up as a sparse linear Group Lasso recovery problem, find sufficient recovery conditions, and demonstrate its effectiveness on data.

==> gradients-jmlr-proofs.tex <==
\section{Recovery guarantees for \flasso}
\label{sec:flassorecovery}

We now give recovery guarantees for the (\flasso) problem. The
guarantees are deterministic, but they depend on the noise sample
covariance, hence they can lead to statistical guarantees holding
w.h.p. in the usual way. The first theorem deals with support recovery, proving that all coefficients outside the support are zeroed out, under conditions that depend only on the dictionary, the true support $S$ and the noise.  The second result completes the previous with error bounds on the estimates $\bhat_j$, assuming an additional condition on the magnitude of the true $\beta_j$ coefficients. Since these coefficients are partial derivatives w.r.t. the dictionary functions, the condition implies that the the dependence on each function must be strong enough to allow the accurate estimation of the partial derivatives.

Introduce the following quantities
\beq \label{eq:mu}
\text{$S$-incoherence in $\G$}\quad \mu\;=\;\max_{i=1:n,j\in S,j'\not\in S}|x_{ij}^Tx_{ij'}|\,
\eeq
\beq
\text{noise level $\sigma$ defined by}\quad \sum_{i=1}^n||\epsilon_i||^2=nd\sigma^2,
\eeq
and {\em internal colinearity $\nu$}, defined as follows. Let 
\beq\label{eq:Sigma}
\Sigma_i\;=\;\left[x_{ij}^Tx_{ij'}\right]_{j,j'\in S}=\;\xb^T_{tS}\xb_{iS},
\quad 
\text{and}
\quad\Sigma\;=\;\diag\{\Sigma_{1:n}\}
\eeq
and  denote by $\nu\leq 1$ the maximum eigenvalue of $\Sigma^{-1}$; a smaller $\nu$ means that the $x_{ij}$ gradients are closer to being orthogonal at each datapoint $i$. 
\begin{theorem}[Support recovery]\label{thm:S} Assume that equation \eqref{} holds, and that $||x_{ij}||=1$ for all $i=1:n,j=1:p$. Denote by $\bbar$ the solution of \eqref{eq:flasso} for some $\lambda>0$.
If $\mu\nu \sqrt{s}+\frac{\sigma \sqrt{nd}}{\lambda}<1$, then $\bbar_{tj}=0$ for $j\not \in S$.
\comment{$y_i\;=\;\xb_i\beta_i+w_i\in \rrr^d$ with $E[w_i]=0,Var(w_i)=\sigma^2$.}
\end{theorem}

{\bf Proof} 
We structure equation \eqref{eq:} in the form
\beq
y\;=\;\barbx \bbar^* +\barw
\quad\text{with }y=[y_i]_{i=1:n}\in\rrr^{nd},\;
\bbar=[\beta_i]_{i=1:n}\in\rrr^{np},\;
\eeq
$\tilde{X}_{ij}\in\rrr^{nd}$ is obtained from $x_{ij}$ by padding with zeros for the entries not in the $i$-th segment, $\barbx_j=[[\tilde{X}_{tj}]_{j=1:p}]_{i=1:n}\in \rrr^{nd\times np}$, and $\barbx_j=[\tilde{X}_{ij}]_{i=1:n}\in \rrr^{nd\times n}$ collects the colums of $\barbx$ that correspond to the $j$-th dictionary entry. Note that 
\beq
\tilde{X}_{tj}^T\tilde{X}_{tj'}\;=\;x_{ij}^Tx_{ij'}
\quad \text{and} \quad
\tilde{X}_{tj}^T\tilde{X}_{t'j'}\;=\;0\text{ whenever }t\neq t'.
\eeq
The proof is by the {\em Primal Dual Witness} method, following \cite{elyaderani},what was his inspiration}. 
It can be shown \cite{} that $\bbar$ is a solution to (\flasso) iff, 
\text{for all $j=1:p$},
\beq \label{eq:kkt0} 
\barbx_j^T\barbx(\bbar -\bbar^*)-\barbx_j^T\barw+\lambda z_j\;=\;0\;\in\rrr^n
\text{ with }z_j=\frac{\beta_j}{||\beta_j||}
\text{ if }\beta_j\neq 0 \text{ and $||z_j||<1$ otherwise}.
\eeq
The matrix $\barbx_j^T\barbx$ is a diagonal matrix with $n$ blocks of size $1\times p$, hence the first term in \eqref{eq:kkt0} becomes 
\beq
[ x_{ij}^T\xb_i(\bbar_{i:}-\bbar_{i:}^*)]_{i=1:n}\in \rrr^{n}.
\eeq
Similarly $\barbx_j^T\barw=[x_{ij}^Tw_i]_{i=1:n}\in \rrr^n$.

We now consider the solution $\bhat$ to problem \eqref{eq:} (\flasso) under the additional constraint that $\beta_{tj'}=0$ for $j'\not \in S$. In other words, $\bhat$ is the solution we would obtain if $S$ was known. Let $\zhat$ be the optimal dual variable for this problem, and let $\zhat_S=[\zhat_j]_{j\in S}$. 

We will now complete $\zhat_S$ to a $z\in \rrr^{np}$ so that the pair $(\bhat, z)$ satisfies \eqref{eq:kkt0}. If we succeed, then we will have proved that $\bhat$ is the solution to the original \flasso~problem, and in particular that the support of $\bhat$ is included in $S$. 

From \eqref{eq:kkt0} we obtain values for $z_j$ when $j\not \in S$.
\beq\label{eq:zjcomp}
z_j\;=\;\frac{-1}{\lambda}\barbx_j^T\left[\barbx^T(\bhat-\bbar^*)-\barw\right].
\eeq
In the same time, if we consider all $j\in S$, we obtain from \eqref{eq:kkt0} that $\barbx_S=[\barbx_j]_{j\in S}$ (here the vectors $\beta_S,\beta_S*$ and all other vectors are size $ns$, with entries sorted by $j$, then by $i$). 
\beq \label{eq:beta-err}
\barbx_S^T\barbx_S(\bhat_S-\beta_S^*)-\barbx_S^T\barw+\lambda \zhat_S\;=\;0.
\eeq
Solving for $\bhat_S-\beta_S^*$ in  \eqref{eq:betaerr}, we obtain
\beq
\bhat_S-\beta_S^*\;=\;(\barbx_S^T\barbx_S)^{-1}\left(\barbx_S^T\barw-\lambda \zhat_S\right)\;=\;\Sigma^{-1}\left(\barbx_S^T\barw-\lambda \zhat_S\right).
\eeq 
After replacing the above in \eqref{eq:zjcomp} we have
\beq \label{eq:zj2}
z_j\;=\;\frac{-1}{\lambda}\barbx_j^T\left[\barbx_S\Sigma^{-1}\barbx^T_Sw-\barbx_S\Sigma^{-1}\lambda \zhat_S-\barw\right]
\;=\;\barbx_j^T\barbx_S\Sigma^{-1}\zhat_S+\frac{1}{\lambda}\barbx_j^T(I-\barbx_S\Sigma^{-1}\barbx_S^T)\barw.
\eeq
Finally, by noting that $\Pi=I-\barbx_S\Sigma^{-1}\barbx_S^T$ is the projection operator on the subspace $\range(\barbx_S)^\perp$, we obtain that 
\beq \label{eq:zj}
z_j\;=\;(\barbx_j^T\barbx_S)\Sigma^{-1}\zhat_S+\frac{1}{\lambda}\barbx_j^T\Pi\barw,
\quad\text{for $j\not\in S$}.
\eeq
We must show that $||z_j||<1$ for $j\not\in S$. 
To bound the first term, we note that $\barbx_j^T\barbx_S$ is $n\times ns$, block diagonal, with blocks of size $1\times s$, and with all non-zero entries bounded in absolute value by $\mu$. Hence, for any vector $v=[v_i]_{i=1:n}\in \rrr^{ns}$, $||\barbx_j^T\barbx_Sv||^2=||[(x^T_{ij}x_{iS})v_i]_{i=1:n}||^2=\sum_{i=1}^n||(x^T_{ij}x_{iS})v_i||^2\leq 2\mu^2\sum_{i=1}^n||v_i||^2=\mu^2||v||^2$. But in our case $v=\Sigma^{-1}\zhat_S$, hence $||v||\leq ||\Sigma^{-1}||||\zhat_S||=\nu\sqrt{s}$. 

To bound the second term, we note that $||\barbx_j||=||x_{ij}||=1$, and that $||\Pi \barw||\leq ||\barw||$ because $\Pi$ is a projection. Hence, the norm squared of this term is bounded above $\sum_{i=1}^n||w_i||^2||x_{ij}||^2/\lambda^2=nd\sigma^2/\lambda^2$. 

Replacing these bounds in \eqref{eq:zj} we obtain that 
\beq
||z_j||\leq ||\barbx_j^T\barbx_S\Sigma^{-1}\zhat_S||+||\frac{1}{\lambda}\barbx_j^T\Pi\barw||
\,\leq\, \mu\nu\sqrt{s}+\frac{\sigma \sqrt{dn}}{\lambda}
\;\text{for any $j\not \in S$}.
\eeq
\hfill$\Box$

\begin{theorem}\label{thm:beta} Assume that equation \eqref{} holds, and that $||x_{ij}||=1$ for all $i=1:n,j=1:p$. Denote by $\bhat$ the solution to problem (\flasso) for some $\lambda>0$. If (1) $\mu\nu \sqrt{s}<1$, (2) $\lambda=(c-1)\sigma\sqrt{dn}$ with $c>1+\frac{1}{1-\mu\nu\sqrt{s}}$, (3) $||\beta_j^*||>c\sigma\sqrt{dn}(1+\sqrt{s})$ for all $j\in S$, then the support $S$ is recovered exactly and $||\bhat_j-\beta^*_j||<c\sigma\sqrt{dn}(1+\sqrt{s})$ for all $j\in S$.
\end{theorem}

{\bf Proof} According to Theorem \ref{thm:S}, $\bhat_j=0$ for $j\not \in S$. It remains to prove the error bound for $j\in S$. According to Lemma V.2 of \cite{elyaderani:}, for any $j\in S$,
\beqa
||\bhat_j-\beta^*_j||
&\leq &||\barbx_j^T\barw||+||\barbx_S^T\barw||+\lambda(1+\sqrt{s})\\
&\leq &(||\barbx_j||+||\barbx_S||)||\barw||+\sigma(c-1)\sqrt{dn}(1+\sqrt{s})\\
&\leq &(1+\sqrt{s})\sigma\sqrt{dn}+\sigma(c-1)\sqrt{dn}(1+\sqrt{s})
\;=\;c\sigma\sqrt{dn}(1+\sqrt{s})
\eeqa
Hence, if $||\beta_j^*||>c\sigma\sqrt{dn}(1+\sqrt{s})$, $\bhat_j\neq 0$ and the support is recovered. 
\hfill $\Box$

Note that for this value of $c$, $\frac{\sigma\sqrt{dn}}{\lambda}+\mu\nu\sqrt{s}=\frac{1}{c-1}+\mu\nu\sqrt{s}<1$.

The assumptions we make are not probabilistic, while those in \cite{elyaderani,} are. In spite of this difference, the assumptions in our work bear comparison with \cite{}. Specifically, our conditions only concern the internal collinearity, for functions  $j\in S$, while \cite{elyaderani} requires bounds on the {\em intra-block coherence} (the equivalent condition) for the whole dictionary. Second, we only require incoherence between $g_S$ and the functions not in $S$; this property is most similar to the {\em inter-block coherence} bound from \cite{elyaderani}. In other words, we show that incoherence between functions outside the support is not necessary. This conclusion can be extended in a straightforward manner to other group Lasso recovery proofs. 


==> gradients-jmlr-replicates.tex <==




\paragraph{Ethanol}\label{sec:ethanol}

%Ethanol has no p-orbital hybridization, and a more intricate vibrational structure than toluene.
Figure \ref{fig:molecs} shows that the estimated manifold is a two-dimensional toroidal surface, and that the two generators of the torus corresponds to bond torsions $g_1$ and $g_2$.  Our dictionary consists of these two torsions, as well as two other dihedral angles. \ouralg~ identifies that $g_1$ and $g_2$ explain the manifold. Furthermore, it associates $g_1$ with embedding coordinates $\phi_1$ and $\phi_2$ and $g_2$ with $\phi_3$, which reflects the orientation of the generators in the Figure.

%
\begin{figure}[H]
\setlength{\picwi}{0.3\llw}
\begin{tabular}{ccc}
\includegraphics[width=4\picwi,height=1.5\picwi]{../Figures/ethanol/June_27_2019_17_17_08/betassymlogsymlogbeta_paths_n50000nsel100nreps5.png}
\end{tabular}
\caption{\ethdata~ The left panel displays $||\beta_{1:p}||$ as a function of the regularization parameter $\lambda$. The remaining panels display, each for one of the embedding coordinates $\phi_k$, the norm of the vector $\vec(\beta_{i,j,k},\,i=1:n')$. For $\lambda > 10^4$, $\phi_{1,2}$ are explained by $g_1$, while $\phi_3$ is explained by $g_2$. Note that some preference is given to $g_2$ by $\phi_3$, and that this corresponds to the embedding that we see in Figure \ref{fig:molecs}. Axes are linear between $0$ and $1$, and logarithmic above $1$. Error bars summarize the outcomes of the $\omega$ repetitions.
}
\label{fig:mds-ethanol}  
\end{figure}

\paragraph{Malonaldehyde}\label{sec:malonaldehyde}

\begin{figure}[H]
\setlength{\picwi}{0.3\llw}
\begin{tabular}{ccc}
\includegraphics[width=4\picwi,height=1.5\picwi]{../Figures/malonaldehyde/June_27_2019_17_24_21/betassymlogsymlogbeta_paths_n50000nsel50nreps5.png}
\end{tabular}
\caption{\maldata~ The left panel displays $||\beta_{1:p}||$ as a function of the regularization parameter $\lambda$. The remaining panels display, each for one of the embedding coordinates $\phi_k$, the norm of the vector $\vec(\beta_{i,j,k},\,i=1:n')$. For $\lambda > 10^2$, $\phi_{1,2,3}$ are explained by $g_{1:2}$. This corresponds to the embedding that we see in Figure \ref{fig:molecs}. Axes are linear between $0$ and $1$, and logarithmic above $1$. Error bars summarize the outcomes of the $\omega$ repetitions.
\label{fig:mds-malonaldehydel} }
\end{figure}

%Malonaldehyde has a slightly more complex structure than ethanol, with possible p-orbital hybridization between the two oxygen atoms.

Figure \ref{fig:molecs} shows that the estimated manifold is a two-dimensional surface on which bond torsions $g_1$ and $g_2$ vary smoothly. Our dictionary consists of these two torsions, as well as two other dihedral angles. \ouralg~ identifies that $g_1$ and $g_2$ explain the manifold. In contrast to ethanol and rigid ethanol, all coordinates are associated indistinguishably with both functions.

%\mmp{to merge if needed}

\paragraph{Toluene}\label{sec:toluene}
%Toluene is a simple small molecule with one rotational degree of freedom.  P-orbital hybridization keeps the benzene ring and its peripheral hydrogens locked in a planar configuration, while the CH3 methyl group can rotate freely.

Figure \ref{fig:molecs} shows that the estimated manifold is a circle parameterized by the $CH_3$ methyl torsion $g_1$.  Our dictionary consists of this angle, as well as other dihedral angles throughout the molecule. \ouralg~  identifies that $g_1$ explains the manifold, and associates both coordinates with this function. 
 It is easy
to see that the the \dpullalg~maps tangent vectors from the embedding
space back to the correct subspace.

%In contrast to the setting in the previous section, we have no a priori knowledge of the shape of the data manifold. We can visually check that this circle corresponds to a bond torsion of the methyl group.

%\ouralg~ provide a statistically validated alternative to this visual inspection method.
\begin{figure}[H]
\setlength{\picwi}{0.3\llw}
\begin{tabular}{ccc}
\includegraphics[width=4\picwi,height=1.5\picwi]{../Figures/toluene/June_27_2019_17_17_08/betassymlogsymlogbeta_paths_n50000nsel50nreps5.png}
\end{tabular}
\caption{\toldata~ The left panel displays $||\beta_{1:p}||$ as a function of the regularization parameter $\lambda$. The remaining panels display, each for one of the embedding coordinates $\phi_k$, the norm of the vector $\vec(\beta_{i,j,k},\,i=1:n')$. For $\lambda > 10^3$, $\phi_{1,2}$ are explained by $g_{1}$. This corresponds to the embedding that we see in Figure \ref{fig:molecs}. Axes are linear between $0$ and $1$, and logarithmic above $1$. Error bars summarize the outcomes of the $\omega$ repetitions.
}
\label{fig:mds-toluene}

